ArtEmis: Affective Language for Visual Art

We present a novel large-scale dataset and accompanying machine learning models aimed at providing a detailed understanding of the interplay between visual content, its emotional effect, and explanations for the latter in language. In contrast to most existing annotation datasets in computer vision, we focus on the affective experience triggered by visual artworks and ask the annotators to indicate the dominant emotion they feel for a given image and, crucially, to also provide a grounded verbal explanation for their emotion choice. As we demonstrate below, this leads to a rich set of signals for both the objective content and the affective impact of an image, creating associations with abstract concepts (e.g., "freedom" or "love"), or references that go beyond what is directly visible, including visual similes and metaphors, or subjective references to personal experiences. We focus on visual art (e.g., paintings, artistic photographs) as it is a prime example of imagery created to elicit emotional responses from its viewers. Our dataset, termed ArtEmis, contains 439K emotion attributions and explanations from humans, on 81K artworks from WikiArt. Building on this data, we train and demonstrate a series of captioning systems capable of expressing and explaining emotions from visual stimuli. Remarkably, the captions produced by these systems often succeed in reflecting the semantic and abstract content of the image, going well beyond systems trained on existing datasets. The collected dataset and developed methods are available at https://artemisdataset.org.

==> sections/scratch.tex <==
## NOTES.

#1. paragraph use (e.g., at results vs. \paragraph{\noindent {\bf XX.}} } 
how much talking about the same emotion makes the language more similar?
    \item \panos{is space allows: add a small vignette with images where people all agree emotionally, fear vs. happiness to highlight the trend.}
    \item \leo{it maybe interesting to ask if subjects that respond with the same emotion to a painting do so for the same reasons or not.}
    \item \mohamed{Perhaps it is nice to provide more details (e.g., top nouns and verbs for every emotion?)} \panos{yes! we have some of that based on PMI but I think due to space it will go to the appendix.}
    \item \mohamed{mohamed:  It would be nice to offer a simple figure to show speaker architectures either in main paper or appendix if we do not have a space}. \panos{have this in mind for appendix - thanks! }
\end{itemize}


%%% ABSTRACT

%\begin{abstract}
%We present a novel large-scale dataset and accompanying machine learning models aimed at providing a detailed understanding of the interplay between visual content, its emotional effect, and explanations for the latter in language. In contrast to most existing visio-linguistic works, we focus on the affective experience triggered by visual artworks and curate responses that indicate the dominant emotion humans feel at their sight, and, crucially, accompany their subjective emotional reactions with visually grounded linguistic explanations. As we demonstrate below, this leads to a very rich signal for both the objective and the affective or semantic content of an image, associating it with abstract concepts (e.g., ``freedom'' or ``love''), or references that go beyond what is directly visible, including visual similes or metaphors. We focus on visual art (e.g., paintings, artistic photographs) as it is a prime example of imagery created to elicit emotional reactions to its viewer. Our dataset, termed \textit{\datasetname}, contains  \numcaptionsshort~emotion explanations from humans, on a large set of artworks from WikiArt. Building on this data, we a train and demonstrate a series of captioning systems capable of expressing and explaining emotions from visual stimuli. Remarkably, the captions produced by these systems often succeed in reflecting the semantic and abstract content of the image, going well-beyond systems trained on existing datasets.
%\end{abstract}

% Previous version
% % !TEX root = ../main.tex
% \begin{abstract}
%  % The relationship of images and human language has been a major topic in computer vision research, as language is a key tool for getting to the semantics of visual inputs, providing supervision for learning algorithms, enabling image search, allowing conversational agents, etc.
%  Much of the extant computer vision work on the relationship between images and human language has focused on literal descriptions of the content of images in terms of objects depicted or actions observed. A certain class of images, however, generates human affective responses which have a strong (and prized) semantic significance well beyond a basic understanding of the scene or action -- and which can also be studied via language.  Visual art (e.g., paintings, artistic photographs) is a prime example of imagery created to elicit emotional responses from the viewer. We hypothesize that neural networks can be built that emulate humans when generating and explaining emotions triggered by visual content, such as 2D artwork. Towards this end, we have built a unique and large-scale captioning dataset, termed \textit{\datasetname}, containing  \numcaptionsshort~emotion explanations from humans, elicited by a large variety of 2D artworks from WikiArt. In building \datasetname~we ask subjects to indicate the dominant emotion they feel at the sight of the stimulus and, crucially, to also provide a grounded verbal explanation for their choice. We find that i) while the emotions expressed are to a certain degree subjective and user-dependent, there is enough common-ground in them that image-classifiers can learn from, ii) human emotion explanations contain far richer language than traditional captioning systems, leading to longer and more varied utterances, frequently using abstract concepts (e.g., ``freedom'' or ``love''), or references that go beyond what is directly visible in an image, such as similes or metaphors. Building on a study of these utterances and their structure, we a create and demonstrate a series of neural-speakers capable of expressing and explaining emotions from visual stimuli. Interestingly, our best performing models make emotion selections and explanation productions that fare well in common captioning (machine-induced) metrics, and more importantly in relevant human-studies, demonstrating progress towards an emotional Turing test.
%  \end{abstract}
 
 % Version 0.
%  In this work we hypothesize and demonstrate that building neural networks that can speak like humans do when explaining emotions that might be triggered at the sight of emotionally charged visual content and particularly, 2D artwork, is feasible. To investigate our hypothesis we first build a large scale unique captioning dataset termed \textit{\datasetname}~that contains \numcaptionsshort~emotion explanations of humans, produced at the sight of a large variety of 2D artwork from WikiArt. In building \datasetname~we ask human subjects to both indicate the dominant emotion they feel at the sight of a given stimulus, and crucially, to also provide a grounded verbal explanation for their choice. By analyzing \datasetname~we note some critical aspects of the underlying cognitive process for explaining emotions that we exploit when we build neural-speakers and when we create relevant evaluation metrics. Specifically, we find that i) while the emotions felt are to a large degree subjective and user-dependent there is enough common-ground in them that image-classifiers can learn from, ii) human explanations contain rich language using frequently abstract concepts (e.g., freedom or love), and reference that goes beyond what is directly visible in an image, e.g., they contain similes ($>20\%$ of the time), and iii) the collected explanations tend to be linguistically more similar when they concern the same emotion. \mohamed{todo: make sure that this experimentally validates and comment with some numbers} We tap on each of these properties and build a series of neural-speakers that reflect them either in their structural bias (e.g., a neural-speaker that is grounded, or not- with a desired emotion), or via the used training data (e.g., training speakers with objective-language only). Interestingly, our best performing models make productions that fare well in common captioning (machine-induced) metrics, and more importantly in relevant human-studies. I.e., they utter explanations that are considered human-made \todo{AMT-study missing} of the time; verifying this way our posed hypothesis.\mohamed{add possible contrast between old school vs new school captioning methods.}
%%% END ABSTRACT

%%% Related Work
% \paragraph{Neuroscience theories of emotion.} The \emph{Theory of Constructed Emotions} is a  scientific theory in Neuroscience by Lisa Feldman Barrett~\cite{barrett2017emotions,barrett2017theory,barrett2006solving,barrett2007mice} that aims to explain the perception and experience  of emotion, arguing that emotions are learned and not genetically endowed. The theory argues that emotions are instantiated by our perception and experience in ways that we can often explain and justify.  Our {\datasetname} is in line with this recent neuroscience research, as we ask human subjects for an explanation of the emotion they experience when viewing an artistic piece.  

%%% END Related Work


% Explanation of emotions raised at the sight of emotionally charged visual representations is key cognitive human process. Building intelligent systems  that learns to generalize on this task opens an exciting new direction in human-computer communication and interaction. In this paper we take the first step in this direction by focusing on linguistic \textit{explanations} and visual artworks with abundant emotion-provoking content. We build a large scale relevant dataset, \datasetname~ and create a set of neural agents (speakers) that show promising performance on this task.

% \paragraph{Discussion} The $C_{emotion|explanation}$ can be easily modified to also take as input the image associated with the provided explanation. We observe minimal gains by doing this in terms of the attained prediction accuracy. \panos{obviously I will reshape and drop most of the following} This is important, as it suggests that the additionally provided visual cues are either not easy to learn or (more likely) that the textual information provides already `enough' clues for solving the task. It is also reasonable to believe this, since we know that the exist very high variance in the choices (classes) humans make given an image. This fact also makes the learning task of $C_{emotion|image}$ challenging.  However, keep in mind that (a) there do exist visual cues or entire painting-subcategories that are for instance significantly more likely to raise positive emotional responses than negative, and (b), it would be reasonable to have a subset of our images annotated by more than 5 humans, e.g., have something closer to 20, which we could use for training and validation purposes. 

% see It is no accident that people have devised hand gestures, make faces, or modulate their vocal tone in order to better convey their emotions and mood \todo{add citations}.


% See supplemental for a detailed analysis of the something-else listed emotions. 


% \item from "The Art Instinct: Beauty, Pleasure, and Human Evolution" (Denis Dutton): "“Kenya and Iceland—what can be more different in the whole fucking world—and both want blue landscapes.” "“The emotions felt by our distant ancestors toward advantageous landscapes are of little use to us today, since we are no longer nomadic hunters who survive off the land. Nevertheless, since we still have souls of those ancient nomads, these emotions can flood into modern minds with surprising and unexpected intensity.” "“ Emotions function in this way, “orchestrating” the mind’s many subprograms so they function smoothly together. They give the example of fear. This emotion, taking hold of a person who walking at night in a potential “stalking and ambush” situation” “In particular, the attraction of natural savanna-like scenes can be increased by signs of human habitation—control and intervention. The preferred areas of low grasses may appear to have been grazed by domestic stock. A road going distance can increase appeal, or a cottage with smoke curling from the chimney. Such post-Pleistocene signs of settlement or agriculture have become clichés in calendar or greeting-card art perhaps they seem to humanize a landscape, rendering it less threatening.”


% \subsubsection{Emotion Classification}
% \begin{enumerate}
% \item $C_{emotion|explanation}$ is text classifier that takes as input a user explanation and learns to map it to one of the nine user-provided options (eight types of emotions, or `something-else').
% \item $C_{emotion|image}$ is an image classifier that is trained to minimize the KL-divergence between its output and the empirical distribution of user-made choices regarding their emotional, or not, reaction for a given image (recall that we have at least, but also on average, five human judgments per image).
% \end{enumerate}


% \textit{``art is a human activity consisting in this, that one man consciously, by means of certain external signs, hands on to others feelings he has lived through, and that other people are infected by these feelings, and also experience them"}~\cite{tolstoy-art}. 

	
% 	\item Last, we show that our best neural speakers make productions that fare well per common captioning (machine-induced) metrics, and more importantly in relevant human-studies. I.e., they utter explanations that are considered human-made \todo{} of the time; verifying this way our posed hypothesis.
% 	\item With separate human studies we verify that the language of \datasetname~is referential w.r.t. the content of the underlying art-work, while expressing subjective opinions, it is sensible as judged by a human listener, and adequate to deduce from it the underlying emotion.
% 	\item We create a variety of neural speakers (\todo{add high-level summary of models}), including speakers which allow us to control the emotional emotional orientation of their production.


% The four positive emotions are finer grained versions of \textit{happiness} which was also proposed by Ekman~\cite{ekman_emotions}, but which as shown later (e.g.,~\cite{happiness}) can have multiple meanings (such as pleasure, life satisfaction, well being, etc.). 

% (as downloaded in 2015) 


% \subsection{Building ArtEmis}
% \todo{expand-explain design choices of Interface} \ref{fig:data_collection_interface}.  
% Facts: 97.5 acceptance rate. We rejected 10,801 submissions. Add also those that we drop for having less than 5 words?. 1.16 years of work from 

% \mohamed{\noindent \textbf{ COCO Data~\cite{lin2014microsoft,coco_chen2015}}   COCO dataset is a seminal work that allowed a significant progress in the computer Vision community. The proper design of the data collection and diligence put in this work is apparent on the quality and its impact  in tasks like Object Detection (e.g., ~\cite{girshick2015fast}), Image-Sentence Retrieval (e.g.,~\cite{vendrov2015order}), and Image Captioning(~\cite{xu2015show,cornia2020meshed}).  In contrast with this curated style of the MS-COCO images, we aim in this work to study emotional language response from  F. Barret's perspective. A key grounding element of COCO dataset collection is the 91 common objects and the objectivity of the captions, `Our dataset contains photos of 91 objects types that would be easily recognizable by a 4 year old.''. Motivated by this comment, we conducted a Human Experiment comparing MS-COCO dataset with the Emotional Responses we collected on WikiArt (one of the largest available collection of Art covering centures of art styles). In particular, we asked ``'Do you think this image description requires a level of emotional/cognitive maturity beyond a 4 year old child?''. The results in \textbf{Fig~\ref{}(TODO: JOINT with TEASER, 77.0\% for ArtEmis, 23.7\% COCO)} is consistent with COCO collection strategy and the contrast shows a key difference compared our collected dataset where we can study our  emotional responses on  centuries of meaningful art and culture images.   } 



% \mohamed{\noindent \textbf{Emotion AI and Theory of Constructed Emotions~\cite{barrett2017emotions,barrett2017theory}:}  Theory of constructed emotions is a relatively recent  scientific theory to explain the perception and experience   of emotion,  proposed by Lisa Feldman Barrett to resolve what she calls the ``emotion paradox''~\cite{barrett2006solving}. The theory challenged the correctness of the current view of Emotion AI systems, which focuses mainly in  recognition of emotion from facial expressions. Theory of constructed emotions claims that emotions are instantiated by our perception and experience that we often can explain and justify. Inspired by this work, we built a dataset where we ask Human Subjects what emotions they have constructed when they experience an artistic piece.% from 3000s BC to 2000s AD. 
% We also them them to explain the constructed emotion. The psychological experiments verified by researched studying this theorems guided the data collection setup of our dataset as we discuss later~\cite{barrett2007mice,barrett2006emotions}. When we measured emotions  of our dataset  to the seminal COCO captions dataset~\cite{lin2014microsoft,coco_chen2015}, we observed both qualitatively and experimentally emotional intensity that is about three times higher shown in Fig.~\ref{fig:teaser2}; (ArtEmis: 77.0 , COCO: 23.7). This results is not surprising duo to not only the domain  difference but also that COCO dataset  is collected on``91 object times that would be easily recognizable by a 4 year old.''~\cite{lin2014microsoft,coco_chen2015}, as the authors  stated.} 


%Emotional response of COCO dataset as not as high is consistent with the statement of the authors  `Our dataset contains photos of 91 objects types that would be easily recognizable by a 4 year old.''.  {TODO: add more citations here. }.       %that gained interest in industry and society.  
%Lisa F. Barret studied  in her seminal work on understanding Human Emotions concluded that Emotions are constructed not triggered in contrary to the classical view of emotions~\cite{barrett2017emotions}. The work concludes decades of research and her theory gained credibility in the scientific community. As we show later in Sec~\ref{YY}, we were inspired by this theory of constructed emotion to design the data collection interface of ArtEmis so that Turkers can more accurately self-identify their emotion. }


% (universal) NLTK tagger




%  Figure~\ref{fig:turing-test} for more details.

% \begin{figure}[t!]
%   \includegraphics[width=\linewidth]{figures/dataset_analysis/turing_test.png}
%   \caption{\textbf{Turing test results.}}
%   \label{fig:turing-test}
% \end{figure}


% See also, \ref{table:c5_vs_c40} for the effect of increasing the replication coverage of each artwork from 5 annotations to 40 on this metrics, for a small random subset of artworks (350 images). \panos{explain the findings}.
% \input{tables/c5_vs_c40_experiment}



%% BELOW is scratch

% For instance, in the previous test-subpopulation of images with strong majority preference no image with the label anger exists (see Sup.Mat for details). Also, interestingly this image2emotion classifier predicts 28.3\% a positive and negative emotion as the two most likely emotions (46.8\% if you count something-else).

% Figure~\ref{appendix:fig:bert_confusion_matrix}). Because of this, if we measure the test accuracy in a simplified/altered label set: \todo{explain} the 3-way classification performance for  is: $YY\%$, $85.6\%$, $89.1\%$, respectively, and for the 2-way $XX\%$, . I.e., all systems are quite successful in recognizing among positive vs. negative emotions.
% e note that both models had adequate capacity to overfit the dataset (near-perfect train-accuracy)\mohamed{reasons for overfitting.?}, and that our final chosen models achieved both better test-error when properly regularized (dropout and early stopping), and had small generalization error (see Supplemental). 
% We test human's and neural-based classifiers' capacity to address this recognition task. After trying this first on AMT — and observing poor performance,  to a visual stimulus
